Driven-dissipative phases and dynamics in non-Markovian nonlinear photonics

Interactions between photons (nonlinearities) enable a powerful form of control over the state of light. This control has enabled technologies such as light sources at new wavelengths, ultra-short optical pulses, frequency-comb metrology systems, even quantum light sources. Common to a wide variety of nonlinear optical technologies is an equilibrium between an energy source, such as an external laser, and dissipation, such as radiation loss or absorption. In the vast majority of these systems, the coupling between the system and the outside world (which leads to loss) is well-described as ``Markovian,'' meaning that the outside world has no memory of its past state. In this work, we introduce a class of driven-dissipative systems in which a nonlinear cavity experiences non-Markovian coupling to the outside world. In the classical regime, we show that these non-Markovian cavities can have extremely low thresholds for nonlinear effects, as well as self-pulsing instabilities at THz rates, and rich phase diagrams with alternating regions of stability and instability. In the quantum regime, we show how these system, when implemented on state-of-the-art platforms, can enable generation of strongly squeezed cavity states with intensity fluctuations that can be more than 15 dB below the classical limit, in contrast to the Markovian driven-dissipative cavity, in which the limit is 3 dB. In the regime of few-photon nonlinearity, such non-Markovian cavities can enable a deterministic protocol to generate Fock states of high order, which are long-desired, but still elusive at optical frequencies. We expect that exploiting non-Markovian couplings in nonlinear optics should in the future lead to even richer possibilities than those discussed here for both classical and quantum light manipulations.

==> preamble.tex <==
%-----CHANGING CITATION APPEARANCE----
\setcitestyle{numbers,square,sort&compress} %We don't want the rmp citation style, but standard style square bracket, numbers style instead

%----KERNING-----
\usepackage{microtype} %For better kerning and symbol-stretching
\usepackage{xspace} %For the \xspace command

%----LOADING RELEVANT FONTS [TIMES ROMAN FOR PRB] -----
\usepackage{txfonts}  %Times Roman fonts
\usepackage{txfontsb} %Addition for txfonts, including old style numerals and greek
%					  %\usepackage{mathptmx} Also a Times Roman Font
%\usepackage{bm} %Bold math symbols with \bm{} (Greek and other symbols)
%\usepackage{mnsymbol} %For llangle and rrangle

%-----CROSS-REFERENCING-----
\usepackage{xr}

%-----COLOR AND GRAPHICS PACKAGES-----
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{tikz}
\usetikzlibrary{calc,decorations.markings}

%-----SETTINGS FOR REFERENCES-----
\usepackage{hyperref}
\hypersetup{
    colorlinks,
    linkcolor={blue!75!black!80!yellow},
    citecolor={blue!75!black!80!yellow},
    urlcolor={blue!75!black!80!yellow}
}

%-----PACKAGE FOR BOXED MULTI-LINE EQUATIONS-----
\usepackage{empheq}
\newcommand*\widefbox[1]{\fbox{\hspace{2em}#1\hspace{2em}}}

%-----CHANGE MARGINS OF DOCUMENT-----
\usepackage[top=1in, bottom=1.5in, left=1.4in, right=1.4in]{geometry} %Change margins

%-----SOME SETTINGS FOR MARGINPAR-----
%\usepackage{marginfix} %Should fix even more than mparhack, so use this instead unless you see something funky

\let\oldmarginpar\marginpar %This and the next line changes the fontsize
\def\marginpar#1{\oldmarginpar{\scriptsize #1}}
\setlength{\marginparwidth}{6.5em} %Changes the width of the note
\setlength{\marginparsep}{2em} %Probably enforces a minimum distance between marginpar-notes


%INCLUDING CLEVEREF PACKAGE FOR MORE CONVENIENT REFERENCING ABILITIES
\usepackage[capitalize,nameinlink]{cleveref}
\newcommand{\crefrangeconjunction}{\,--\,}
\crefname{subequations}{Eqs.}{Eqs.} %Specific changes to allow for Eqs.-wording when referring to a set of subequations. Label of subequations must include [subequations] as an option.
\Crefname{subequations}{Eqs.}{Eqs.}
\crefformat{subequations}{#2Eqs.~(#1)#3}
\Crefformat{subequations}{#2Eqs.~(#1)#3}
\crefname{page}{p.}{p.} %Changing from 'page' to 'p.'
\newcommand{\heqref}[1]{\hyperref[#1]{(\ref*{#1})}} %Alternative to \eqref, which works better with hyperlinks (whole thing is clickable)
\newcommand{\namedref}[2]{\hyperref[#2]{#1~\ref*{#2}}} %\nameref{Name}{label} will produce Name~\ref{label} with the entire thing clickable
\newcommand{\namedeqref}[2]{\hyperref[#2]{#1~(\ref*{#2})}} %\nameref{Name}{label} will produce Name~\ref{label} with the entire thing clickable


%-----PACKAGE TO ALLOW CHANGING OF ENUMERATE BULLETS-----
\usepackage{enumitem}

%-----COMMANDS-----
\newcommand{\vek}[1]{\mathbf{#1}}
\newcommand{\rv}{\mathbf{r}}
\newcommand{\qv}{\mathbf{q}}
\newcommand{\kv}{\mathbf{k}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\nablav}{\boldsymbol{\nabla}}
\newcommand{\hxv}{\hat{\mathbf{x}}}
\newcommand{\hyv}{\hat{\mathbf{y}}}
\newcommand{\ef}{\epsilon_{\text{\textsc{f}}}}
\newcommand{\vf}{v_{\text{\textsc{f}}}}
\newcommand{\tsc}[1]{\text{\textsc{#1}}}
\newcommand{\kb}{k_\tsc{b}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\ddb}[1]{\!\dd#1\,}
\newcommand{\dde}{\,\dd}
\newcommand{\appropto}{\mathrel{\vcenter{
  \offinterlineskip\halign{\hfil$##$\cr
    \propto\cr\noalign{\kern.2pt}\sim\cr\noalign{\kern-2.5pt}}}}}

\newcommand{\spar}{_{\scriptscriptstyle\parallel}}
\newcommand{\kpar}{k_{\scriptscriptstyle\parallel}}
\newcommand{\kvpar}{\kv_{\scriptscriptstyle\parallel}}
\newcommand{\rpar}{r_{\scriptscriptstyle\parallel}}
\newcommand{\rvpar}{\rv_{\scriptscriptstyle\parallel}}
\newcommand{\vpar}{v_{\scriptscriptstyle\parallel}}
\newcommand{\vvpar}{\vv_{\scriptscriptstyle\parallel}}
\newcommand{\dperp}{d_{\perp}}
\newcommand{\dpar}{d_{\parallel}}
\newcommand{\iu}{\mathrm{i}}

\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\newcommand{\tr}{\operatorname{Tr}}
\newcommand{\sgn}{\operatorname{sgn}}

\newcommand{\pr}[1]{|#1\rangle\langle#1|}
\newcommand{\prsf}[1]{\mathsf{|#1\rangle\langle#1|}}

\newcommand{\Ev}{\mathbf{E}}
\newcommand{\Dv}{\mathbf{D}}
\newcommand{\Hv}{\mathbf{H}}
\newcommand{\Bv}{\mathbf{B}}
\newcommand{\ev}{\mathbf{e}}
\newcommand{\dv}{\mathbf{d}}
\newcommand{\hv}{\mathbf{h}}
\newcommand{\bv}{\mathbf{b}}
\newcommand{\Gv}{\mathbf{G}}
\newcommand{\Rv}{\mathbf{R}}
\newcommand{\nv}{\hat{\mathbf{n}}}

%abbreviations
\newcommand{\ie}{i.e.\@\xspace} %Gobble-spaces of the "small" type (small is ensured by adding \@)
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\eg}{e.g.\@\xspace}
